Perspective Flow Aggregation for Data-Limited 6D Object Pose Estimation

Most recent 6D object pose estimation methods, including unsupervised ones, require many real training images. Unfortunately, for some applications, such as those in space or deep under water, acquiring real images, even unannotated, is virtually impossible. In this paper, we propose a method that can be trained solely on synthetic images, or optionally using a few additional real ones. Given a rough pose estimate obtained from a first network, it uses a second network to predict a dense 2D correspondence field between the image rendered using the rough pose and the real image and infers the required pose correction. This approach is much less sensitive to the domain shift between synthetic and real images than state-of-the-art methods. It performs on par with methods that require annotated real images for training when not using any, and outperforms them considerably when using as few as twenty real images.

==> figs/flow_geometry.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    % \begin{tabular}{cc}
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/1.png} &
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/2.png} \\
    % (a) & (b) \\
    % \end{tabular}
    % \fbox{\rule{0pt}{2in} \rule{\linewidth}{0pt}}
    % 
    % https://tex.stackexchange.com/questions/16519/adding-space-between-columns-in-a-table
    \addtolength{\tabcolsep}{-5pt}  % whose value is usually 6pt
    \begin{tabular}{cccc}
    \includegraphics[width=0.8\linewidth]{./figs/placeholder.png}
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000002_0005.jpg}&
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000018_0010.jpg}&
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000003_0054.jpg}\\
    % \includegraphics[width=0.24\linewidth,trim=250 200 250 300,clip]{./fig/motivation/scene_000022_0000.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=300 300 300 300,clip]{./fig/motivation/scene_000002_0005.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=500 420 350 430,clip]{./fig/motivation/scene_000018_0010.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=420 450 480 450,clip]{./fig/motivation/scene_000003_0054.jpg}\\
%     3d & 8d & 20d & 30d \\
    \end{tabular}
    \addtolength{\tabcolsep}{5pt}  % restore previous value
    % 
    \end{center}
    \vspace{-6mm}
    \caption{{\bf The flow geometry.} bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla blabla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla }
    \label{fig:flow_geom}
\end{figure}


==> figs/refinement_comp.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    % \begin{tabular}{cc}
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/1.png} &
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/2.png} \\
    % (a) & (b) \\
    % \end{tabular}
    % \fbox{\rule{0pt}{2in} \rule{\linewidth}{0pt}}
    % 
    % https://tex.stackexchange.com/questions/16519/adding-space-between-columns-in-a-table
    \addtolength{\tabcolsep}{-5pt}  % whose value is usually 6pt
    \begin{tabular}{cccc}
    \includegraphics[width=0.8\linewidth]{./figs/refinement_comp/comp.pdf}
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000002_0005.jpg}&
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000018_0010.jpg}&
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000003_0054.jpg}\\
    % \includegraphics[width=0.24\linewidth,trim=250 200 250 300,clip]{./fig/motivation/scene_000022_0000.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=300 300 300 300,clip]{./fig/motivation/scene_000002_0005.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=500 420 350 430,clip]{./fig/motivation/scene_000018_0010.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=420 450 480 450,clip]{./fig/motivation/scene_000003_0054.jpg}\\
%     3d & 8d & 20d & 30d \\
    \end{tabular}
    \addtolength{\tabcolsep}{5pt}  % restore previous value
    % 
    \end{center}
    \vspace{-6mm}
    \caption{{\bf The flow geometry.} bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla blabla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla }
    \label{fig:flow_geom}
\end{figure}


==> figs/render_3dpoint.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    % \begin{tabular}{cc}
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/1.png} &
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/2.png} \\
    % (a) & (b) \\
    % \end{tabular}
    % \fbox{\rule{0pt}{2in} \rule{\linewidth}{0pt}}
    % 
    % https://tex.stackexchange.com/questions/16519/adding-space-between-columns-in-a-table
    \addtolength{\tabcolsep}{-5pt}  % whose value is usually 6pt
    \begin{tabular}{ccc}
    \includegraphics[width=0.3\linewidth]{./figs/render_3dpoint/1.png} &
    {\setlength{\fboxsep}{-0.5pt}\setlength{\fboxrule}{0.5pt}\fbox{\includegraphics[width=0.3\linewidth]{./figs/render_3dpoint/2.png}}} &
    {\setlength{\fboxsep}{-0.5pt}\setlength{\fboxrule}{0.5pt}\fbox{\includegraphics[width=0.3\linewidth]{./figs/render_3dpoint/3.png}}} \\
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000002_0005.jpg}&
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000018_0010.jpg}&
%     \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000003_0054.jpg}\\
    % \includegraphics[width=0.24\linewidth,trim=250 200 250 300,clip]{./fig/motivation/scene_000022_0000.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=300 300 300 300,clip]{./fig/motivation/scene_000002_0005.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=500 420 350 430,clip]{./fig/motivation/scene_000018_0010.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=420 450 480 450,clip]{./fig/motivation/scene_000003_0054.jpg}\\
%     3d & 8d & 20d & 30d \\
    (a) & (b) & (c) \\
    \end{tabular}
    \addtolength{\tabcolsep}{5pt}  % restore previous value
    % 
    \end{center}
    \vspace{-6mm}
    \caption{{\bf Inferring 3D object points during rendering.} {\bf (a)} is a rendered image. {\bf (b)} shows the corresponding 3D object points. {\bf (c)} shows the same 3D object points in a different view. Given the 3D mesh, for every 2D pixel on the rendered target, we infer its corresponding 3D object point by a ray-mesh intersection algorithm.~\cite{1}. \YH{Maybe duplicated with Fig.~\ref{fig:flow_examplar}}}
    \label{fig:render_3dpoint}
\end{figure}

